SpecRover: Code Intent Extraction via LLMs

Autonomous program improvement typically involves automatically producing bug fixes and feature additions. Such program improvement can be accomplished by a combination of large language model (LLM) and program analysis capabilities, in the form of an LLM agent. Since program repair or program improvement typically requires a specification of intended behavior - specification inference can be useful for producing high quality program patches. In this work, we examine efficient and low-cost workflows for iterative specification inference within an LLM agent. Given a GitHub issue to be resolved in a software project, our goal is to conduct iterative code search accompanied by specification inference - thereby inferring intent from both the project structure and behavior. The intent thus captured is examined by a reviewer agent with the goal of vetting the patches as well as providing a measure of confidence in the vetted patches. Our approach SpecRover (AutoCodeRover-v2) is built on the open-source LLM agent AutoCodeRover. In an evaluation on the full SWE-Bench consisting of 2294 GitHub issues, it shows more than 50% improvement in efficacy over AutoCodeRover. Compared to the open-source agents available, our work shows modest cost ($0.65 per issue) in resolving an average GitHub issue in SWE-Bench lite. The production of explanation by SpecRover allows for a better "signal" to be given to the developer, on when the suggested patches can be accepted with confidence. SpecRover also seeks to demonstrate the continued importance of specification inference in automated program repair, even as program repair technologies enter the LLM era.

==> background.tex <==
\section{Background}

\paragraph{Repository-level issue solving}

Repository-level issue solving refers to the task of automatically finding a solution to issues in real-world large software repositories.
The issues usually only contain a natural language description, and can be either bug fixing or feature addition to the codebase.
Repository-level issue solving is a challenging tasks, because (1) it requires the understanding of a large codebase, (2) the problem description is in natural language which can be vague, and (3) it requires identifying the code relevant to the problem description from the large codebase in order to make code modifications.

Various benchmarks have been proposed to study the problem of repository issue solving, such as X~\cite{}, Y~\cite{}, and Z~\cite{}. Among the benchmarks, SWE-Bench~\cite{jimenez2024swebench} is currently the most commonly used. It consists of 2294 GitHub issues collected from well-known Python projects. For each issue, an issue-resolving tool is given as input the issue statement and the buggy project version on which the issue was reported. The tool is supposed to produce a patch to resolve the issue. The produced patch is then evaluated with a set of acceptance tests. Note that some of the acceptance tests are not accessible to the issue-resolving tool when producing the patch, because they were only added to the involved project after the issue was reported.

\paragraph{AutoCodeRover}

AutoCodeRover~\cite{} is one of the earliest and state-of-the-art repository-level issue resolving techniques. The main idea of AutoCodeRover is to glean program specification from the structure of the program. Unlike many other issue-resolving techniques, which view the program as a mere collection of files, AutoCodeRover views the program as a syntax tree and autonomously explores the tree to understand the program. This exploration process is called \emph{context retrieval} in AutoCodeRover. After the context retrieval, AutoCodeRover performs patch generation with the gleaned specification. 

\paragraph{Program Repair}

Program repair~\cite{} studies the problem of automatically fixing bugs in a program. It is closely related to issue resolving, as many issues require bug fixing. The major difference between program repair and issue resolving lies in the representation of the involved bug. In program repair, the bug is usually witnessed by one or more failing test cases, and the goal of repair is to make the program pass these tests. On the contrary, issue-resolving techniques do not assume the availability of failing test cases. Instead, only a natural-language description of a fault is provided to represent the bug.

%Program repair techniques fall in two main categories: search-based~\cite{} and constraint-based~\cite{}. Search-based program repair techniques try to find a correct patch via random search. In contrast, constraint-based program repair first infers symbolic constraints needed to pass the failing test cases, and then synthesizes a patch satisfying the constraints. Essentially, the inferred symbolic constraint is a representation of the program specification. 

==> figures/table-review-stat.tex <==
\begin{table}[h!]
\label{tab:review-stat}
\centering
\caption{Breakdown of reviewer decisions. }
\begin{tabular}{r|cccc}
\toprule
\multirow{2}{*}{Type} & \multicolumn{2}{c|}{Correcrt Test} & \multicolumn{2}{c}{Incorrect Test} \\
\cmidrule{2-3} \cmidrule{4-5}
 & \multicolumn{1}{c|}{Pass} & \multicolumn{1}{c|}{Fail}  & \multicolumn{1}{c|}{Pass} & \multicolumn{1}{c}{Fail} \\ 
\midrule
TP & X & Y & Z & W \\
TN & ... &  \\
FP & &  \\
FN & &  \\
\midrule
Total & & \\
\bottomrule
\end{tabular}
\end{table}

==> figures/table-wrong-review.tex <==
\begin{table}[h!]
\label{tab:wrong-review}
\centering
\caption{Reasons for incorrect reviewer decisions on SWE-Bench lite. }
\begin{tabular}{ll}
\toprule
Reason & \# Tasks \\
\midrule
Misleading Reproducer Test & X\% \\ 
Changed Regression Test  & Y\% \\
Wrong Review & \\ 
\midrule
Total & Z \\
\bottomrule
\end{tabular}
\end{table}

==> method_angelic.tex <==
\subsection{Angelic Value: Specification from Test}

Another specification effectively leveraged by \toolname is the angelic value. The angelic value of a selected expression in the program is a value that can rescue a failing test case, i.e., replacing the expression with the value will make the test case pass. In essence, the angelic value is the specification in the test case extracted at a particular program location.

The angelic value makes a useful complement to the aforementioned function summary. Specifically, the function summary captures the general program specification at the function level. By intuition, the summary will help an LLM agent keep the general program semantics and avoid regression. In contrast, the angelic value represents a specification that is test-specific, or rather issue-specific, and at the expression level. Therefore, the angelic value will be more helpful in instructing the agent to rectify the defect related to the issue. In fact, the angelic value underpins a number of techniques for program rectification, e.g., angelic debugging~\cite{} and semantic program repair~\cite{}.

Despite its usefulness in rectifying programs, the use of angelic value for LLM programming agents is largely unexplored. The most related work is \cite{parasaram2024factselectionproblemllmbased}, which shows that angelic values can help the LLM fix certain bugs. However, this approach cannot be applied in practice, because it obtains angelic values by executing a program that is already fixed, which is unavailable in practice.
%Besides, they use the angelic value of each and every variable, which can be difficult to compute. 
Meanwhile, the standard way of computing angelic values, which is symbolic execution followed by constraint solving~\cite{},
% TODO: elaborate on constraint solving
relies on a mature symbolic execution engine, which is unavailable for some programming languages, e.g., Python and JavaScript.

In this study, we propose the first practical method to obtain and leverage angelic values for an LLM programming agent. To obtain angelic values, we send queries to an LLM, which contain expression values recorded during a failed test execution as well as a prompt requesting for angelic values. In response, the LLM will provide angelic values to rescue the execution.

The benefit of querying an LLM for angelic values is twofolds. First, this approach does not rely on a symbolic execution engine, making it more versatile than the standard symbolic execution approach. More importantly, the LLM is able to provide the angelic value for more types of expressions, compared to symbolic execution. Specifically, symbolic execution can mainly deal with integer and boolean types, while the LLM can provide a description of any type of expression. This versatility in terms of data types is especially useful for high-level programming languages, e.g., Python and JavaScript, which involve complex objects.
% TODO: this sentence is abrupt
We do note that the description given by an LLM may not be as precise as a value computed via symbolic execution. However, the description is good enough for guiding our patching agent, as shown in our experiment.

A sample query for angelic values and the response from the LLM are shown in Figure~\ref{}. As shown in the figure, a query starts with a \emph{buggy trace}, which is the values of some selected expressions at every program location within a single function. These values are recorded during a failed test execution. After giving the buggy trace, the query prompts the LLM to provide an \emph{angelic trace} containing values that can rescue the test execution. Finally, to produce a more succinct description of the angelic values so as to guide the patching agent more effectively, we prompt the LLM to summarize the difference between the buggy trace and the angelic trace. The buggy trace, angelic trace, and summary will be passed to the patching agent for reference.

To compose such a query, it needs to be decided which function and what expressions within the function to track. Both decisions are made via an LLM. The LLM is provided with the issue statement, buggy locations found by the context retrieval agent, and the stacktrace and the error information of the reproducer test. For deciding the function, we use an LLM to choose from the buggy locations. By constraining the choice within these buggy locations, we are able to make sure that the chosen function is relevant to the issue. After deciding the function to track, we prompt the LLM to choose expressions in the function to track. The LLM is often able to choose one or more problematic expressions, given the stacktrace and the error information of the reproducer test, as observed in our experiment. 
